Group Invariant Dictionary Learning

The dictionary learning problem concerns the task of representing data as sparse linear sums drawn from a smaller collection of basic building blocks. In application domains where such techniques are deployed, we frequently encounter datasets where some form of symmetry or invariance is present. Motivated by this observation, we develop a framework for learning dictionaries for data under the constraint that the collection of basic building blocks remains invariant under such symmetries. Our procedure for learning such dictionaries relies on representing the symmetry as the action of a matrix group acting on the data, and subsequently introducing a convex penalty function so as to induce sparsity with respect to the collection of matrix group elements. Our framework specializes to the convolutional dictionary learning problem when we consider integer shifts. Using properties of positive semidefinite Hermitian Toeplitz matrices, we develop an extension that learns dictionaries that are invariant under continuous shifts. Our numerical experiments on synthetic data and ECG data show that the incorporation of such symmetries as priors are most valuable when the dataset has few data-points, or when the full range of symmetries is inadequately expressed in the dataset.

==> sec_numsimplifications.tex <==
%\section{Specialization of Proposition \ref{thm:atomicnorm_fullsdp} for Learning Continuously Shift Invariant Dictionaries.} \label{sec:ctsshift_implementation}

\subsubsection{Implementation details} \label{sec:ctsshift_implement}

In the following, we explain how Proposition \ref{thm:atomicnorm_fullsdp} is applied within our dictionary learning framework.  Let $\by \in \R^{2d+1}$ be the data vector and let $\{\ba_i\}_{i=1}^{q} \in \R^{2d+1}$ be generators for the dictionary.  Let $\tilde{\by}:= F \by$ and $\tilde{\ba}_i := F \ba_i$ be the data and the generator expressed in the transformed basis, and let $\odot$ denote pointwise multiplication.  Then the loss can be re-written as follows: $\| \by - \sum_{i} \left( F^{\dagger} L(\phi) F \right) \ba_i \|_2^2 = \| (F \by) - \sum_{i} L(\phi) (F \ba_i) \|_2^2 =  \| \tilde{\by} - \sum_{i} l(\phi) \odot \tilde{\ba}_i \|_2^2$.

Following Proposition \ref{thm:atomicnorm_fullsdp}, the step in which we represent $\by$ as succinctly with respect to $\mathcal{D}$ as in \eqref{eq:atomicnorm_sparsecoding} is given by:
\begin{equation} \label{eq:ctsshiftsparsecoding}
\begin{aligned}
& \underset{\substack{ z_{i,+},z_{i,-} \in \R,\\ \bz_{i,+},\bz_{i,-} \in \mathbb{C}^{d}}}{\mathrm{argmin}} \frac{1}{2} \| \tilde{\by} - \sum_{i=1}^{q} \tilde{\ba}_i \odot (
\left(\begin{array}{c}
\bz_{i,+}^{\ast} \\ z_{i,+} \\ \bz_{i,+} 
\end{array}\right)
-
\left(\begin{array}{c}
\bz_{i,-}^{\ast} \\ z_{i,-} \\ \bz_{i,-}
\end{array}\right)
) \|_2^2  \\
& \qquad\qquad\qquad\qquad\qquad\qquad + \lambda \sum_{i=1}^{q} (z_{i,+} + z_{i,-}) \\
&  \mathrm{s.t.}
\left( \begin{array}{cc}
z_{i,+} & \bz_{i,+}^{\dagger} \\
\bz_{i,+} & \star
\end{array}\right),
\left( \begin{array}{cc}
z_{i,-} & \bz_{i,-}^{\dagger} \\
\bz_{i,-} & \star
\end{array}\right) \text{are PSD Toeplitz}
\end{aligned}.
\end{equation}

